Unlocking the Latent Canvas: Eliciting and Benchmarking Symbolic Visual Expression in LLMs

Current multimodal approaches predominantly treat visual generation as an external process, relying on pixel rendering or code execution, thereby overlooking the native visual representation capabilities latent within Large Language Models (LLMs). In this work, we unlock this potential through ASCII art, a compact, efficient, and text-native visual format. We introduce SVE-ASCII, a unified framework designed to elicit and benchmark Symbolic Visual Expression directly within the pure text space. To address the scarcity of systematic resources, we construct ASCIIArt-7K, a high-quality dataset synthesized via a novel "Seed-and-Evolve" pipeline that augments human-curated anchors through in-context stylistic editing. We further implement a unified instruction-tuning strategy that jointly optimizes for both Generation (Text-to-ASCII) and Understanding (ASCII-to-Text). Crucially, our experiments reveal a critical phenomenon regarding task duality: while it is established that perception aids generation, we provide compelling evidence that generative training significantly enhances visual comprehension. This confirms a mutually reinforcing cycle in symbolic visual processing, a relationship previously hypothesized but rarely empirically demonstrated in the visual domain. We release our dataset, the ASCIIArt-Bench benchmark, and the SVE-ASCII model, establishing a robust baseline for native text-based visual intelligence.

==> tables/table4.tex <==
\begin{table*}[htbp]
    \centering
    \caption{\textbf{User Study of ASCII-Mix Model and baselines.}}
    \label{tab:user_study}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Method} & \textbf{Prompt Alignment $\uparrow$} & \textbf{Visual Quality $\uparrow$} & \textbf{Pick Score $\uparrow$} \\
        \midrule
        GPT-4o \cite{0}   & 0  & 0  & 0  \\
        Gemini-3.0-Flash \cite{0}  & 0  & 0  & 0  \\
        Gemini-2.5-Flash \cite{0}  & 0  & 0  & 0  \\
        Doubao-Pro \cite{0}  & 0  & 0  & 0  \\
        Qwen-2.5-72B \cite{0}  & 0  & 0  & 0  \\
        DeepSeek-V3 \cite{0} & 0  & 0  & 0  \\
        Qwen2.5-7B-Instruct (Base) \cite{0}   & 0  & 0  & 0  \\
        \textbf{ASCII-Mix (Ours)}   & \textbf{0} & \textbf{0} & \textbf{0} \\
        \bottomrule
    \end{tabular}
\label{tab:table4}
\end{table*}
